Self-Correcting Large Language Models: Generation vs. Multiple Choice

Large language models have recently demonstrated remarkable abilities to self-correct their responses through iterative refinement, often referred to as self-consistency or self-reflection. However, the dynamics of this self-correction mechanism may differ substantially depending on whether the model is tasked with open-ended text generation or with selecting the most appropriate response from multiple predefined options. In this paper, we conduct a systematic investigation of these two paradigms by comparing performance trends and error-correction behaviors across various natural language understanding and reasoning tasks, covering language models of different scales and families. Our experimental results reveal distinct patterns of improvement and failure modes: \textit{While open-ended generation often benefits from the flexibility of re-interpretation and compositional refinement, multiple-choice selection can leverage clearer solution boundaries but may be limited by the provided options}. This contrast also reflects the dual demands faced by emerging agentic LLM applications: effective agents must not only generate and refine open-ended plans or explanations, but also make reliable discrete choices when operating within constrained action spaces. Our findings, therefore, highlight that the design of self-correction mechanisms should take into account the interaction between task structure and output space, with implications for both knowledge-intensive reasoning and decision-oriented applications of LLMs.

==> tables/tab_sample_3.tex <==
\begin{table*}[ht]
\centering
\caption{tinyTruthfulQA - Llama3.1-8B - Baseline}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cp{7cm}p{7cm}}
\toprule
\rowcolor{gray!5}
\textbf{Question} & \multicolumn{2}{l}{-} \\
\midrule
\rowcolor{gray!5}
& \textbf{Generation Answer} & \textbf{MCQ Answer} \\
\midrule
% \rowcolor{lightgreen}
\rowcolor{green!10}
\textbf{Answer} & - & - \\
\midrule
0 & - & - \\
\midrule
1 & - & - \\
\midrule
2 & - & - \\
\midrule
3 & - & - \\
\midrule
4 & - & - \\
\midrule
5 & - & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

